On Differentially Private U Statistics

We consider the problem of privately estimating a parameter $\mathbb{E}[h(X_1,\dots,X_k)]$, where $X_1$, $X_2$, $\dots$, $X_k$ are i.i.d. data from some distribution and $h$ is a permutation-invariant function. Without privacy constraints, standard estimators are U-statistics, which commonly arise in a wide range of problems, including nonparametric signed rank tests, symmetry testing, uniformity testing, and subgraph counts in random networks, and can be shown to be minimum variance unbiased estimators under mild conditions. Despite the recent outpouring of interest in private mean estimation, privatizing U-statistics has received little attention. While existing private mean estimation algorithms can be applied to obtain confidence intervals, we show that they can lead to suboptimal private error, e.g., constant-factor inflation in the leading term, or even $\Theta(1/n)$ rather than $O(1/n^2)$ in degenerate settings. To remedy this, we propose a new thresholding-based approach using \emph{local H\'ajek projections} to reweight different subsets of the data. This leads to nearly optimal private error for non-degenerate U-statistics and a strong indication of near-optimality for degenerate U-statistics.

==> macros.tex <==
\usepackage[english]{babel}
\usepackage[utf8x]{inputenc}
\usepackage[T1]{fontenc}
\usepackage{algorithm,bbm}
\usepackage{algorithmic}
\usepackage{xcolor}
%\setlength\parindent{0pt}
\usepackage{amsmath}
\usepackage{amssymb,mathtools,verbatim}
\usepackage{amsthm}

% \usepackage[a4paper,top=3cm,bottom=2cm,left=3cm,right=3cm,marginparwidth=1.75cm]{geometry}
%\usepackage{amsthm}
% The following packages will be automatically loaded:
% amsmath, amssymb, natbib, graphicx, url, algorithm2e
\newtheorem{theorem}{Theorem}
\newtheorem{lemma}{Lemma}
\newtheorem{fact}{Fact}
\newtheorem{definition}{Definition}

\newtheorem{corollary}{Corollary}
\newtheorem{proposition}{Proposition}
\newtheorem{conjecture}{Conjecture}
\newtheorem{remark}{Remark}
\newtheorem{setting}{Setting}


\newcommand{\tvect}[2]{
   \ensuremath{\Bigl(\negthinspace\begin{smallmatrix}#1\\#2\end{smallmatrix}\Bigr)}}
\newcommand{\rd}{\color{red}}
\newcommand{\bk}{\color{black}}
\newcommand{\bone}{\mathbbm{1}}
\newcommand{\I}{\mathcal{I}}
\newcommand{\defeq}{:=}
\newcommand{\norm}[1]{\left\lVert#1\right\rVert}
\newcommand{\norms}[1]{\lVert#1\rVert}
\newcommand{\normop}[1]{\left\lVert#1\right\rVert_{\textup{op}}}
\newcommand{\normf}[1]{\left\lVert#1\right\rVert_{\textup{F}}}
\newcommand{\normtr}[1]{\left\lVert#1\right\rVert_{\textup{tr}}}
\newcommand{\normsop}[1]{\lVert#1\rVert_{\textup{op}}}
\newcommand{\norminf}[1]{\lVert#1\rVert_{\infty}}
\newcommand{\normsf}[1]{\lVert#1\rVert_{\textup{F}}}
\newcommand{\inprod}[2]{\left\langle#1, #2\right\rangle}
\newcommand{\inprods}[2]{\langle#1, #2\rangle}
\newcommand{\eps}{\epsilon}
\newcommand{\lam}{\lambda}
\newcommand{\E}{\mathbb{E}}
\renewcommand{\P}{\mathbb{P}}
\newcommand{\clip}{\textsf{clip}}
% \newcommand{\argmax}{\textup{argmax}}
% \newcommand{\argmin}{\textup{argmin}} 
\newcommand{\R}{\mathbb{R}}
\newcommand{\C}{\mathbb{C}}
\newcommand{\N}{\mathbb{N}}
\newcommand{\bas}[1]{\begin{align*}#1\end{align*}}
\newcommand{\ba}[1]{\begin{align}#1\end{align}}
\newcommand{\bbb}[1]{\left[#1\right]}
\newcommand{\bmb}[1]{\left | #1\right |}
\newcommand{\bcb}[1]{\left \{ #1\right \}}
\newcommand{\diag}[1]{\textbf{\textup{diag}}\left(#1\right)}
\newcommand{\half}{\frac{1}{2}}
\newcommand{\thalf}{\tfrac{1}{2}}
\newcommand{\1}{\mathbbm{1}}
%\newcommand{\E}{\mathbb{E}}
\newcommand{\Var}{\textup{Var}}
\newcommand{\Vol}{\textup{Vol}}
\newcommand{\Nor}{\mathcal{N}}
\newcommand{\smax}{\textup{smax}}
\newcommand{\smin}{\textup{smin}}
\newcommand{\Tr}{\textup{Tr}}
\newcommand{\opt}{\textup{OPT}}
\newcommand{\xset}{\mathcal{X}}
\newcommand{\yset}{\mathcal{Y}}
\newcommand{\zset}{\mathcal{Z}}
%\newcommand{\set}{\mathcal{K}}
\newcommand{\ball}{\mathbb{B}}
\newcommand{\ma}{\mathbf{A}}
\newcommand{\ai}{\ma_{i:}}
\newcommand{\aj}{\ma_{:j}}
\newcommand{\id}{\mathbf{I}}
\newcommand{\bb}[1]{\left(#1\right)}
\newcommand{\jac}{\mathbf{J}}
\newcommand{\dd}{\textup{d}}
\newcommand{\nk}{n_k}
%\newcommand{\bas}[1]{\begin{align*}#1\end{align*}}
\usepackage{xcolor}
\newcommand{\tn}{\hat{\theta}_{\text{naive}}}
\newcommand{\tall}{\tilde{\theta}_{\text{all}}}
\newcommand{\tss}{\hat{\theta}_{\text{ss}}}
\newcommand{\tpss}{\tilde{\theta}_{\text{ss}}}
\newcommand{\varfactor}{\frac{1}{\sqrt{\alpha}}}
\newcommand{\Varfactor}{\varfactor}
\newcommand{\succprob}{1-O\bb{\alpha}}

\definecolor{color1}{rgb}{0.8, 0.33, 0.0}
\definecolor{color2}{rgb}{0.0, 0.3, 0.9}
\newcommand{\shourya}[1]{\textcolor{color1}{\textbf{shourya:} #1}}
\newcommand{\purna}[1]{\textcolor{color2}{\textbf{purna:} #1}}
\newcommand{\G}{\mathcal{G}}
\newcommand{\proj}{\text{proj}}
\newcommand{\tO}{\widetilde{O}}
\newcommand{\nnz}{\textup{nnz}}
\newcommand{\Prox}{\textup{Prox}}
\newcommand{\Par}[1]{\left(#1\right)}
\newcommand{\Brack}[1]{\left[#1\right]}
\newcommand{\Brace}[1]{\left\{#1\right\}}
\newcommand{\Abs}[1]{\left|#1\right|}
\newcommand{\Cov}{\textup{Cov}}
\newcommand{\oracle}{\mathcal{O}}
\newcommand{\alg}{\mathcal{A}}
\newcommand{\mproj}{\mathbf{P}}
\newcommand{\mm}{\mathbf{M}}
\newcommand{\mb}{\mathbf{B}}
\newcommand{\mv}{\mathbf{V}}
\newcommand{\msig}{\boldsymbol{\Sigma}}
\newcommand{\mlam}{\boldsymbol{\Lambda}}
\newcommand{\tmlam}{\widetilde{\mlam}}
\newcommand{\tmsig}{\widetilde{\msig}}
\newcommand{\ms}{\mathbf{S}}
\newcommand{\ml}{\mathbf{L}}
\newcommand{\tms}{\widetilde{\ms}}
\newcommand{\tml}{\widetilde{\ml}}
\newcommand{\mmu}{\mathbf{U}}
\newcommand{\mr}{\mathbf{R}}
\newcommand{\mq}{\mathbf{Q}}
\newcommand{\var}{\text{var}}
\newcommand{\Good}{\text{Good}}
\newcommand{\Bad}{\text{Bad}}
\newcommand{\conc}{\xi}
\newcommand{\cc}{\mathcal{C}}
\newcommand{\hj}{Hájek }
% \newcommand{\buf}[1]{\xi_{#1}}
\newcommand{\buf}[1]{L_{#1}}
\newcommand{\proxy}{\tau}
\newcommand{\X}{\mathbf{X}}
\newcommand{\F}{\mathcal{F}}
\newcommand{\dep}[3]{\text{dep}_{#1,#2}\bb{#3}}
% \newcommand{\h}[3]{\hat{h}^{#1}_{1}({#3})}
% \newcommand{\g}[3]{\hat{g}^{#1}_{1}({#3})}
\newcommand{\h}[3]{\hat{h}_{#1}({#3})}
\newcommand{\g}[3]{\hat{g}_{#1}({#3})}
\newcommand{\Yc}[1]{Q(#1)}
\newcommand{\Uc}[1]{Q^{\text{avg}}(#1)}
\newcommand{\varup}{\sigma_{\text{max}}}
\newcommand{\varlo}{\sigma_{\text{min}}}
\newcommand{\A}{\mathcal{A}}
\newcommand{\haj}[2]{\hat{h}_{#1}\bb{#2}}
\newcommand{\wt}{\text{wt}}
\newcommand{\covar}{\text{cov}}

\DeclareMathOperator{\polylog}{polylog}
\DeclareMathOperator*{\argmin}{\arg\min}
\DeclareMathOperator*{\argmax}{\arg\max}
\DeclareMathOperator{\Laplace}{Lap}
\DeclareMathOperator{\Lap}{Lap}
\DeclareMathOperator{\Bernoulli}{Ber}
\DeclareMathOperator{\Ber}{Ber}
% \DeclareMathOperator{\TV}{d\_{TV}}
\newcommand{\SubS}{\mathcal{S}}
\newcommand{\SubA}{A_n}
\newcommand{\tSubA}{\tilde{A}_n}


==> privdegen.tex <==
We design an algorithm that builds upon ideas in \citep{ullman2019er} and exploits the concentration of the Hájek projections $\h{}{X}{i}$ in the case of degenerate U statistics. Let $\conc$ be a parameter to be defined later; this parameter will be set so that with high probability, we have $\bmb{\h{}{X}{i}-\theta} \le \conc$, as in Lemma~\ref{lem:degen_conc_hajek}.
% Let $\sqrt{\tilde{\zeta}_k}$ be an $\epsilon$-differentially private estimate of the variance of $h$. Define
% \[
% \conc \defeq \bb{\sqrt{\frac{4kK}{n}}\sqrt{\tilde{\zeta}_k} + \frac{4k}{3n}C}\log \frac{12n}{\beta}.
% \]
% By Lem~\ref{lem:degen_conc_hajek}, $\conc$ is such that with high probability, all of the projections $\h{}{X}{i}$ are $\conc$-close to the true mean $\theta$.
For any $n$-tuple $\X = (X_1, X_2, \ldots, X_n)$, let 
\ba{\label{eq:Ustat}
U_n(\X) \defeq \frac{1}{\binom{n}{k}} \sum_{S \in \mathcal{I}_{n,k}} h(X_S), \qquad
\h{\X}{X}{i} \defeq \frac{1}{\binom{n-1}{k-1}}\sum_{S \in \mathcal{I}^{i}_{n,k}} h(X_S) ~~ \forall i \in [n],
}
and let $\buf{\X}$ be the smallest positive integer $t$ such that at most $t$ indices $i \in [n]$ satisfy the condition $\left |\h{\X}{X}{i} - U_n(\X) \right | > \conc +\frac{(2k-1)Ct}{n-1}$; such an integer always exists because $t = n$ works. Define
\ba{\label{eq:goodset}
\Good(\X) \defeq \bcb{i : \left |\h{\X}{X}{i}-U_n(\X) \right | \le \conc +\frac{(2k-1)C\buf{\X}}{n-1}}
}
and $\Bad(\X) \defeq [n] \setminus \Good(\X)$.
For each $S \in \mathcal{I}_{n,k}$, define
\bas{
g^{\X}(X_S) \defeq h(X_S)\mathbbm{1}\bb{S \subseteq \Good(\X)} + U_n(\X)\mathbbm{1}\bb{S \not\subseteq \Good(\X)}.
}
Finally, define $\tilde{U}_n(\X)$ and $\g{\X}{X}{i}$ similar to Eq~\ref{eq:Ustat} but replacing the function $h$ with a $g$.
%  and \ba{\label{eq:fg}
% \tilde{U}_n(\X) &\defeq \frac{1}{\binom{n}{k}}\sum_{S \in \mathcal{I}_{n,k}}g^{\X}(X_S), \text{ and} \\
% \g{\X}{X}{i} &\defeq \frac{1}{\binom{n-1}{k-1}} \sum_{S \in \mathcal{I}^{i}_{n,k}} g^{\X}(X_S).
% }

\begin{algorithm}
\caption{\label{alg:PrivateMeanDegenerate} \textbf{PrivateMeanHajek}$\bb{n ,k ,h , \left \{X_i \right\}_{i \in [2n]}, C, \epsilon, \alpha = 0.999}$}
\begin{algorithmic}[1]
{\STATE $\tilde{\zeta}_k \gets $\textbf{PrivateVariance}$\bb{n, k, h, \left \{X_i \right\}_{i \in [n+1,2n]}, C, \epsilon, \alpha}$
\STATE $\conc \gets 2\bb{2\sqrt{\frac{4kK}{n}}\sqrt{\tilde{\zeta}_k} + \frac{4k}{3n}C}\log \frac{12n}{\alpha}$}
\STATE $\X \gets \{X_i\}_{i \in [n]}~ ; ~U_n(\X) \gets \sum_{S \in \mathcal{I}_{n,k}} h(X_S)/\binom{n}{k}$
\FOR{$i = 1,2, \ldots, n$}
\STATE $\h{\X}{X}{i} \gets \sum_{S \in \mathcal{I}^{i}_{n,k}} h(X_S)/\binom{n-1}{k-1}$
\ENDFOR
\STATE Let $\buf{\X}$ be the smallest positive integer such that at most $\buf{\X}$ indices $i$ satisfy $\bmb{\h{\X}{X}{i}-U_n(\X)} > \conc + \frac{(2k-1)C \buf{\X}}{n-1}$
\STATE $\Good(\X) \gets \bcb{i : \bmb{\h{\X}{X}{i}-U_n(\X)} \le \conc + \frac{(2k-1)C \buf{\X}}{n-1}}; \Bad(\X) \gets [n]\setminus \Good(\X)$
\FOR{$S \in \mathcal{I}_{n,k}$}
\STATE $g(X_S) \gets h(X_S)\mathbbm{1}\bb{S \subseteq \Good(\X)} + U_n(\X)\mathbbm{1}\bb{S \not\subseteq \Good(\X)}$
\ENDFOR
\STATE $S(\X) \gets \max_{0 \le \ell \le n} \bb{4k\bb{\buf{\X}+\ell}/n}\bb{2\conc+\bb{17k\bb{\buf{\X}+\ell}C/\bb{n-1}}}e^{-\epsilon \ell}$
\STATE $\tilde{U}_n(\X) \gets \sum_{S \in \mathcal{I}_{n,k}} g(X_S)/\binom{n}{k}$
\RETURN  $\tilde{U}_n(\X) + S(\X)/\epsilon \cdot Z$, where $Z \gets t_3$
\end{algorithmic}
\end{algorithm}

The idea of Algorithm~\ref{alg:PrivateMeanDegenerate} is as follows: If all $\h{\X}{X}{i}$ are within $\conc$ of the mean $U_n(\X)$, then $\Bad(\X) = \varnothing$ and $\tilde{U}_n(\X) = U_n(\X)$. Otherwise, for any $i \in \Bad(\X)$, the quantities $h(X_S)$ are replaced with the empirical mean $U_n(\X)$ of the entire set, for any $i \in S$. As we will show, this averaging-out of the bad indices allows for a bound on the local sensitivity of $\tilde{U}_n$ in terms of $\buf{\X} = \bmb{\Bad(\X)}$, which can be viewed as an indicator of how well-concentrated the data are. We will show that $\buf{\X} = 1$ with high probability, which allows for a good utility guarantee.

\begin{theorem}
Algorithm \ref{alg:PrivateMeanDegenerate} is $2\epsilon$-differentially private. Moreover, if $\zeta_1 = 0$ and $|h|_{\infty} \le C$, then with probability at least $0.99$, we have
\bas{
\bmb{\mathcal{A}(\X) - \theta} = O\bb{\sqrt{\var(U_n)} + 
\frac{k^{3/2} \sqrt{K} \bb{1+1/\epsilon} \log n}{n^{3/2}\epsilon}\sqrt{\zeta_k}  + \frac{k^2 \bb{1+1/\epsilon}^2 \log n}{n^2\epsilon}C}.
}
\end{theorem}

% \begin{lemma}
% $\text{LS}_{\tilde{U}_n}(\X) = O\bb{\frac{r\buf{\X}}{n}\bb{\conc +\frac{Cr\buf{\X}}{n}}}$.
% \end{lemma}

\begin{proof}
The computation of $\tilde{\zeta}_k$ and $\conc$ is $\epsilon$-differentially private. By Lemma~\ref{lem:basic_comp}, it suffices to consider a fixed $\tilde{\zeta}_k$ and show that the rest of the algorithm is $\epsilon$-differentially private. Consider two adjacent datasets $\X = (X_1, X_2, \ldots, X_n)$ and $\X' = (X'_1, X'_2, \ldots, X'_n)$ differing only in the index ${i^*}$, that is, $X'_i = X_i$ for all $i \neq i^*$. Let $B \defeq \Bad(\X ) \cup \Bad(\X ') \cup \{i^*\}$, and let $b \defeq |B|$. Then,
\ba{\label{eq:sum_decomp}
\binom{n}{k}\bb{\tilde{U}_n(\X)-\tilde{U}_n(\X')} %= \sum_{S \in \mathcal{I}_{n,r}}\bb{g^{\X}(X_S)-g^{\X'}(X'_S)} \notag \\
&= \sum_{S \subseteq B^c} \bb{g^{\X}(X_S)-g^{\X'}(X_S')} + \sum_{i \in B} \sum_{S \in \mathcal{I}^{i}_{n,k}} \bb{g^{\X}(X_S)-g^{\X'}(X'_S)} \notag\\
&~~ - \sum_{a=2}^{k} \sum_{\substack{S \in \mathcal{I}_{n,k} \\
\bmb{S \cap B} = a}} (a-1)\bb{g^{\X}(X_S)-g^{\X'}(X'_S)}.
}
The first term in the above equation counts all subsets that are contained in $\Good(\X)\cap \Good(\X ')\setminus \{i^*\}$. The second term now sums over all subsets with an element in $B$. However, this leads to overcounting every subset with $a$ elements in common with $B$ exactly $a-1$ times. The third term corrects for this overcounting akin to an inclusion-exclusion type argument. We will now bound each of the three terms separately.

The first term in Eq~\ref{eq:sum_decomp} is 0; indeed, if $S \subseteq B^c$ then $g^{\X}(X_S) = h^{\X}(X_S) = h^{\X'}(X'_S) = g^{\X'}(X'_S)$. Next, note that
\vspace{-1em}
\ba{\label{eq:Udiff}
\left |U_n(\X) - U_n(\X') \right | = \bmb{\frac{1}{\binom{n}{k}} \sum_{S \in \mathcal{I}^{i^*}_{n,k}}\bb{h(X_S)-h(X'_S)}} \le \frac{kC}{n}.
}
\vspace{-1em}
Next, for any $i \neq {i^*}$,
\ba{\label{eq:hhajekdiff}
\left |\h{\X}{X}{i}-\h{\X'}{X'_i}{} \right | = \bmb{\frac{1}{\binom{n-1}{k-1}} \sum_{S \in \mathcal{I}^{i}_{n,k} \cap \mathcal{I}^{i^*}_{n,k}} \bb{h(X_S)-h(X'_S)}} \le \frac{(k-1)C}{n-1}.
}
Before we bound the other two terms, we make the following crucial claim (proof in Appendix).
\begin{lemma} \label{eq:bufX_sensitivity}
$|\buf{\X}-\buf{\X '}| \le 1.$
\end{lemma}
For any index $i \in [n]$, if $i \notin \Good(\X)$, then $\g{\X}{X}{i} = U_n(\X)$; and if $i \in \Good(\X)$, then
\bas{
\g{\X}{X}{i} &= \frac{1}{\binom{n-1}{k-1}} \sum_{i \in S} h^{\X}(X_S)\mathbbm{1}\bb{S \subseteq \Good(\X)} + \frac{1}{\binom{n-1}{k-1}} \sum_{i \in S} U_n(\X)\mathbbm{1}\bb{S \not\subseteq \Good(\X)} \\
&= \h{\X}{X}{i} + \frac{1}{\binom{n-1}{k-1}} \sum_{i \in S} \bb{U_n(\X) - h(X_S)}\mathbbm{1}\bb{S \not\subseteq \Good(\X)} \\
% &\in\bb{U_n(\X) \pm  \conc  \pm \frac{(2k-1)C\buf{\X}}{n-1}} \pm \bb{\frac{\binom{n-1}{k-1}-\binom{n-1-\buf{\X}}{k-1}}{\binom{n-1}{k-1}}C} \\
}
which implies $|\g{\X}{X}{i} - U_n(\X)| \le\conc  + \frac{(4k-3)C\buf{\X}}{n-1}$. Here, we used
\bas{
\frac{\binom{n-1}{k-1} - \binom{n-1-\buf{\X}}{k-1}}{\binom{n-1}{k-1}} = 1 - \prod_{t=1}^{k-1} \bb{1 - \frac{\buf{\X}}{n-t}} %\le 1 - \bb{1 - \frac{\buf{\X}}{n-k+1}}^{k-1} \\
\le 1 - \bb{1-\frac{\buf{\X}(k-1)}{n-k+1}} \le \frac{2\buf{\X}(k-1)}{n}.
}
% and $\prod_{i=1}^\ell (1-y_i) \ge 1-\sum_{i=1}^\ell y_i$ for any reals $y_1, y_2, \ldots, y_\ell \in (0,1)$.
Either way, $\left |\g{\X}{X}{i} - U_n(\X) \right | \le \conc  + \frac{(4k-3)C\buf{\X}}{n-1},$ so
\ba{\label{eq:ghajekdiff}
\bmb{\g{\X}{X}{i}-\g{\X'}{X'_i}{}} &\le \bmb{U_n(\X)-U_n(\X')} + 2\conc  + \frac{(4k-3)C\buf{\X}}{n-1} + \frac{(4k-3)C\buf{\X'}}{n-1} \notag \\
% &\le \frac{kC}{n} + 2\conc  + \frac{(4k-3)(2\buf{\X}+1)C}{n-1} \notag \\
&\le 2\conc  + \frac{8k\buf{\X}+5k}{n-1}C.
}

Using Eq~\ref{eq:ghajekdiff}, the second term can be bounded as 
\ba{\label{eq:sum_term2}
\bmb{\sum_{i \in B} \sum_{S \in \mathcal{I}^{i}_{n,k}} \bb{g^{\X}(X_S)-g^{\X'}(X'_S)}} &\le \binom{n-1}{k-1} \sum_{i \in B} \bmb{\g{\X}{X}{i} - \g{\X'}{X'_i}{}} \notag \\
&\le \binom{n-1}{k-1}\bb{2\conc  + \frac{8k\buf{\X}+5k}{n-1}C}(2\buf{\X}+2),
}
where we used the fact that $b \le \buf{\X}+\buf{\X'}+1 \le 2\buf{\X}+2$. Finally,
\ba{\label{eq:sum_term3}
&\frac{1}{C}\bmb{ \frac{1}{\binom{n}{k}} \sum_{a=2}^{k} \sum_{\bmb{S \cap B} = a} (a-1)\bb{g^{\X}(X_S)-g^{\X'}(X'_S)}} \le \frac{1}{\binom{n}{k}} \sum_{a=2}^k (a-1)\binom{b}{a}\binom{n-b}{k-a} \notag\\
&= \frac{\binom{n-b}{k}}{\binom{n}{k}} - \bb{1 - \frac{bk}{n}} \le \bb{1 - \frac{b}{n}}^k - \bb{1-\frac{bk}{n}} \le \frac{b^2k^2}{n^2} \le \frac{k^2(2\buf{\X}+2)^2}{n^2}.
}
where we used the identities $\sum_{a=0}^k \binom{b}{a}\binom{n-b}{k-a} = \binom{n}{k}$ and $\sum_{a=0}^k a\binom{b}{a}\binom{n-b}{k-a} = \frac{bk}{n}\binom{n}{k}.$ Combining Eqs~\ref{eq:sum_decomp}, \ref{eq:sum_term2}, \ref{eq:sum_term3}, and the fact that the first term in Eq~\ref{eq:sum_decomp} is zero,
\bas{
\bmb{U_n(\X)-U_n(\X')} %&\le \frac{k(2\buf{\X}+2)}{n}\bb{2\conc  + \frac{(8k-6)\buf{\X}+(5k-3)}{n-1}C} + \frac{(2\buf{\X}+2)^2k^2C}{n^2} \\
&\le \frac{2k(\buf{\X}+1)}{n} \bb{2\conc  + \frac{k\bb{10\buf{\X} + 7}}{n-1}C}
}
which implies that
$LS_{\tilde{U}_n}(\X) \le \frac{4k\buf{\X}}{n} \bb{2\conc  + \frac{17k\buf{\X}}{n-1}C}.
$
%This gives us an upper bound on the local sensitivity of $\tilde{U}_n$ at $\X$ in terms of $\buf{\X}$.
Let $g(\conc ,\buf{\X},n) := \frac{4k\buf{\X}}{n} \bb{2\conc  + \frac{17k\buf{\X}}{n-1}C}$; note that it is strictly increasing in $\buf{\X}$. Define
\ba{\label{eq:smooth_sensitivity}
S(G) = \max_{\ell \in \mathbb{Z}_{\ge 0}} e^{-\epsilon \ell} g(\conc , \buf{\X}+\ell, m).
}
\begin{lemma}\label{lem:smooth_bound}
$S(G)$ is an $\epsilon$-smooth upper bound on $LS_f(G)$. Moreover,
\[S(G) = O\bb{\frac{k\bb{\buf{\X}+1/\epsilon}\bb{\conc  + Ck(\buf{\X}+1/\epsilon)/n}}{n}}.\]
\end{lemma}
% \begin{proof}[Proof of Lemma~\ref{lem:smooth_bound}]
% Clearly, $S(G) \ge g(\conc , \buf{\X}, n) \ge LS_f(G)$, and for any two adjacent $G$ and $G'$,
% \bas{
% S(G') &= \max_{\ell \in \mathbb{Z}_{\ge 0}} e^{-\epsilon \ell} g(\conc , \buf{\X'}+\ell, n) \le \max_{\ell \in \mathbb{Z}_{\ge 0}} e^{-\epsilon \ell} g(\conc , \buf{\X}+\ell+1, n) \\
% &= \max_{\ell \in \mathbb{Z}_{> 0}}e^{-\epsilon \bb{\ell-1}} g(\conc , \buf{\X}+\ell+1, n) \le e^{\epsilon}\max_{\ell \in \mathbb{Z}_{\ge 0}}e^{-\epsilon\ell} g(\conc , \buf{\X}+\ell+1, n) = e^{\epsilon}S(G).
% }
% This shows that $S$ is an $\epsilon$-smooth upper bound on the local sensitivity of $f$. As for the upper bound, for any $\ell \ge 0$, we have
% \bas{
% e^{-\epsilon\ell}g(\conc , \buf{\X}+\ell, n) &= e^{-\epsilon\ell} \frac{4k\bb{\buf{\X}+\ell}}{n} \bb{2\conc  + \frac{17k\bb{\buf{\X}+\ell}}{n-1}C} \\
% &= \frac{4k\bb{\buf{\X}e^{-\epsilon\ell/2}+\ell e^{-\epsilon\ell/2}}}{n} \bb{2\conc  e^{-\epsilon\ell/2} + \frac{17k\bb{\buf{\X}e^{-\epsilon\ell/2}+\ell e^{-\epsilon\ell/2}}}{n-1}C} \\
% &\le \frac{4k\bb{\buf{\X}+1/\epsilon}}{n}\bb{2\conc   + \frac{17k\bb{\buf{\X}+1/\epsilon}}{n-1}C}.
% }
% \end{proof}

By Lemma~\ref{lem:smooth_bound}, it is clear that the term $S(\X)$ added in to $\tilde{U}_n(\X)$ in Algorithm~\ref{alg:PrivateMeanDegenerate} is exactly the smoothed sensitivity defined in Eq~\ref{eq:smooth_sensitivity}. Therefore, the output $\tilde{U}_n(\X)+S(\X)/\epsilon \cdot Z$, where $Z$ is sampled from a Student's $t$-distribution with three degrees of freedom, is $\epsilon$-differentially private. 

\paragraph{Utility.}First, by Chebyshev's inequality, we have with probability at least $1-\alpha$ that
$\bmb{U_n(\X)-\theta} \le \frac{1}{\sqrt{\alpha}}\sqrt{\var(U_n)}.
$
Second, with probability at least $1-\alpha$ the estimate $\tilde{\zeta}_k$ of the variance of $h$ satisfies $\zeta_k \le \tilde{\zeta}_k \le 2\zeta_k$. 
First note that since $\Var(h(X_1,\dots,X_k|X_i)) = \zeta_1 = 0$, we have $\E[h(X_1, \dots, X_k)|X_i] = \E[h(X_1, \dots, X_k)] = \theta$. %Also, since
% $\sigma_i^2  \le \E\bbb{\bb{h(X_S)-\theta}^2|X_i}$

Next, note that $\sigma_i^2$ are IID subexponential random variables with subexponential norm at most $K\zeta_k$, because by Jensen's inequality,
$
\E\bbb{\exp \bb{t\sigma_i^2}} % &= \E\bbb{\exp \bb{t\Var{\bb{h(X_S) | X_1}}}}
%&= \E\bbb{\exp\bb{t \E\bbb{\bb{h(X_S)-\theta}^2 \big| X_1}}} \\
%&\le \E\bbb{\E \bbb{\exp\bb{t \bb{h(X_S)-\theta}^2 } \big| X_1}} \\
\leq \E \bbb{\exp\bb{t \bb{h(X_S)-\theta}^2 } }.
$
Conditioned on this event, and using Lem~\ref{lem:degen_conc_hajek}, with probability at least $1-\alpha$ all $\h{\X}{X}{i}$ satisfy
\vspace{-1em}
\bas{
\bmb{\h{\X}{X}{i}-\theta} \le \bb{2\sqrt{\frac{4kK}{n}}\sqrt{\tilde{\zeta}_k} + \frac{4k}{3n}C}\log \frac{12n}{\alpha} \le \frac{\conc}{2}.
}
\vspace{-.3em}
Moreover, each of the projections $\h{\X}{X}{i}$ is within $\conc/2$ of the true mean $\theta$  with probability at least $1-\alpha$. If so, then each of the projections is also within $\conc$ of the empirical mean of the projections. This means $\Good(\X) = [n]$ and $\buf{\X} = 1$. Also, since all indices are good, $g(X_S) = h(X_S)$ for all $S$ and $\tilde{U}_n(\X) = U_n(\X)$.
Finally, with probability at least $1-\alpha,$ the $Z$ satisfies
$Z \le \frac{1}{\sqrt{\alpha}} \var(t_3) = \frac{3}{\sqrt{\alpha}}.$
Therefore,
\vspace{-1em}
\ba{\label{eq:degen:error}
&\bmb{\mathcal{A}(\X)-\theta} \le \bmb{\tilde{U}_n(\X)-U_n(\X)}+\bmb{U_n(\X)-\theta}+\bmb{S(\X)/\epsilon \cdot Z} \notag\\
%&\le 0 + \frac{1}{\sqrt{\alpha}}\sqrt{\var(U_n)} + \frac{3}{\epsilon \sqrt{\alpha}} \frac{4k\bb{1+1/\epsilon}}{n}\bb{2\conc   + \frac{17k\bb{1+1/\epsilon}}{n-1}C} \\
&= O\bb{\sqrt{\var(U_n)} + 
\frac{k^{3/2} \sqrt{K} \bb{1+1/\epsilon} \log n}{n^{3/2}\epsilon}\sqrt{\zeta_k}  + \frac{k^2 \bb{1+1/\epsilon}^2 \log n}{n^2\epsilon}C}
}
conditioned on all the aforementioned events, which occur with probability $0.99$.
\end{proof}

==> privdegenTAPER.tex <==
We design an algorithm that builds upon ideas in \citep{ullman2019er} and exploits the concentration of the Hájek projections $\h{}{X}{i}$.
% in the case of degenerate U statistics.
Let $\conc$ be a parameter to be defined later; this parameter will be set so that with high probability, we have $\bmb{\h{\X}{X}{i}-\theta} \le \conc$ for all $i$, as in Lemma~\ref{lem:degen_conc_hajek}. For any $n$-tuple $\X = (X_1, X_2, \ldots, X_n)$, let 
\ba{\label{eq:Ustat}
U_n(\X) \defeq \frac{1}{\binom{n}{k}} \sum_{S \in \mathcal{I}_{n,k}} h(X_S)
}
and
\ba{\label{eq:Hajekprojection}
\h{\X}{X}{i} \defeq \frac{1}{\binom{n-1}{k-1}}\sum_{S \in \mathcal{I}^{i}_{n,k}} h(X_S) ~~ \forall i \in [n].
}
Let $\buf{\X}$ be the smallest positive integer $t$ such that at most $t$ indices $i \in [n]$ satisfy the condition $\left |\h{\X}{X}{i} - U_n(\X) \right | > \conc +\frac{2kCt}{n}$; such an integer always exists because $t = n$ works. Define
\ba{\label{eq:goodset}
\Good(\X) \defeq \bcb{i : \left |\h{\X}{X}{i}-U_n(\X) \right | \le \conc +\frac{2kC\buf{\X}}{n}}, \qquad \Bad(\X) \defeq [n] \setminus \Good(\X).
}

We define the distance from an interval as:
\ba{
%\text{proj}(x, \ell, r) &\defeq \argmin_{y \in \bbb{\ell, r}} \bmb{y-x}. \label{eq:proj}\\
\text{dist}(x, \ell, r) &\defeq \min_{y \in \bbb{\ell, r}} \bmb{y-x}. \label{eq:dist}
}
Let $\beta > 0$ be a parameter to be defined later. For each index $i \in [n]$, define
\ba{\label{eq:weight}
\wt^\X(i) \defeq \max\bb{0,1-\beta \text{dist}\bb{\h{\X}{X}{i}, \bbb{U_n-\conc-\frac{2kC\buf{\X}}{n}, U_n+\conc+\frac{2kC\buf{\X}}{n}}}},
}
which is the \textit{weight} of $i$ with respect to the dataset $\X$. Here, $\text{dist}$ refers to the distance function defined in~\eqref{eq:dist}. Intuitively, these weights can be viewed as identifiers of how much the index $i$ should influence the estimate. Define
\ba{\label{eq:set_weight}
\wt^\X(S) = \min_{i \in S} \wt^\X(i) \qquad \forall S \in \I_{n,k},
}
and
\ba{\label{eq:g_def}
g^{\X}(S) \defeq h(X_S)\wt^\X(S) + U_n(\X)\bb{1-\wt^\X(S)}.
}
In particular, if $\wt^\X(S) = 1$ then $g^{\X}(S) = h(X_S)$ and if $\wt^\X(S) = 0$ then $g^{\X}(S) = U_n$. Essentially, we are downweighting the contribution of the bad indices $i$. Finally, define the quantities
\ba{\label{eq:fg}
\tilde{U}_n(\X) \defeq \frac{1}{\binom{n}{k}} \sum_{S \in \mathcal{I}_{n,k}} g^{\X}(S), \qquad
\g{\X}{X}{i} \defeq \frac{1}{\binom{n-1}{k-1}}\sum_{S \in \mathcal{I}^{i}_{n,k}} g^{\X}(S) ~~ \forall i \in [n].
}

\begin{algorithm}
\caption{\label{alg:PrivateMeanDegenerate} \textbf{PrivateMeanHájek}$\bb{n ,k ,h , \left \{X_i \right\}_{i \in [2n]}, C, \epsilon, \alpha = 0.999}$}
\begin{algorithmic}[1]
{\STATE $\tilde{\zeta}_k \gets $\textbf{PrivateVariance}$\bb{n, k, h, \left \{X_i \right\}_{i \in [n+1,2n]}, C, \epsilon, \alpha}$
\STATE $\conc \gets 2\bb{2\sqrt{\frac{4kK}{n}}\sqrt{\tilde{\zeta}_k} + \frac{4k}{3n}C}\log \frac{12n}{\alpha}$}
\STATE $\X \gets \{X_i\}_{i \in [n]}~ ; ~U_n(\X) \gets \sum_{S \in \mathcal{I}_{n,k}} h(X_S)/\binom{n}{k}$
\FOR{$i = 1,2, \dots, n$}
\STATE $\h{\X}{X}{i} \gets \sum_{S \in \mathcal{I}^{i}_{n,k}} h(X_S)/\binom{n-1}{k-1}$
\ENDFOR
\STATE Let $\buf{\X}$ be the smallest positive integer such that at most $\buf{\X}$ indices $i$ satisfy $\bmb{\h{\X}{X}{i}-U_n(\X)} > \conc + \frac{2kC \buf{\X}}{n}$
\STATE $\Good(\X) \gets \bcb{i : \bmb{\h{\X}{X}{i}-U_n(\X)} \le \conc + \frac{2kC \buf{\X}}{n}}; \Bad(\X) \gets [n]\setminus \Good(\X)$
\FOR{$i = 1,2,\dots, n$}
\STATE $\wt^\X(i) \gets \max\bb{0,1-\beta\text{dist}\bb{\h{\X}{X}{i},\bbb{U_n-\conc-\frac{2kC\buf{\X}}{n}, U_n+\conc+\frac{2kC\buf{\X}}{n}}}}$
\ENDFOR
\FOR{$S \in \mathcal{I}_{n,k}$}
\STATE $g^{\X}(S) \gets h(X_S) \min_{i \in S} \wt^\X(i)
+ U_n(\X)\bb{1-\min_{i \in S} \wt^\X(i)}$
\ENDFOR
\STATE $S(\X) \gets \max_{0 \le \ell \le n} e^{-\epsilon \ell}\bb{4k\bb{\buf{\X}+\ell}/n}\bb{2\conc+\bb{17k\bb{\buf{\X}+\ell}C/\bb{n-1}}}$
\STATE $\tilde{U}_n(\X) \gets \sum_{S \in \mathcal{I}_{n,k}} g^{\X}(S)/\binom{n}{k}$
\RETURN  $\tilde{U}_n(\X) + S(\X)/\epsilon \cdot Z$, where $Z \gets t_3$ \footnote{$t_3$ is the Student's t-distribution with three degrees of freedom} 
\end{algorithmic}
\end{algorithm}

The idea behind Algorithm~\ref{alg:PrivateMeanDegenerate} is as follows: If all $\h{\X}{X}{i}$ are within $\conc$ of the mean $U_n(\X)$, then $\Bad(\X) = \varnothing$ and $\tilde{U}_n(\X) = U_n(\X)$. Otherwise, for any $i \in \Bad(\X)$, the quantities $h(X_S)$ care replaced with a weighted combination of $h(X_S)$ and the empirical mean $U_n(\X)$ of the entire set, for any $i \in S$. This averaging-out of the bad indices allows for a bound on the local sensitivity of $\tilde{U}_n$ in terms of $\buf{\X} = \bmb{\Bad(\X)}$, which can be viewed as an indicator of how well-concentrated the data is. The choice of $\conc$ will be such that $\buf{\X} = 1$ with high probability so that the local sensitivity (and the smooth sensitivity) of the estimator at $\X$ is small.

\begin{theorem}\label{thm:mainthm}
Algorithm \ref{alg:PrivateMeanDegenerate} is $2\epsilon$-differentially private. Moreover, if $\zeta_1 = 0$ and additive range at most $C$, then with probability at least $0.99$, we have 
\bas{
\bmb{\mathcal{A}(\X) - \theta} = O\bb{\sqrt{\Var(U_n)} + 
\frac{k^{3/2} \sqrt{K} \bb{1+1/\epsilon} \log n}{n^{3/2}\epsilon}\sqrt{\zeta_k}  + \frac{k^2 \bb{1+1/\epsilon}^2 \log n}{n^2\epsilon}C}.
}
\begin{proof}

\end{proof}
\end{theorem}



==> privdegen_proof_full.tex <==
\begin{proof}
\textcolor{red}{Much of this proof should be appendicized.} The computation of $\tilde{\zeta}_k$ is $\epsilon$-differentially private. By Basic Composition (Lemma~\ref{lem:basic_comp}), it suffices to consider a fixed $\conc$ and show that the rest of the algorithm is $\epsilon$-differentially private. Consider two adjacent datasets $\X = (X_1, X_2, \ldots, X_n)$ and $\X' = (X'_1, X'_2, \ldots, X'_n)$ differing only in the index $i^*$, that is, $X'_i = X_i$ for all $i \neq i^*$.

Let $B \defeq \bb{\Bad(\X ) \cup \Bad(\X ')} \setminus \{i^*\}$ and $G \defeq \bb{\Good(\X ) \cap \Good(\X ') } \setminus \{i^*\}$. Then,
\ba{\label{eq:sum_decomp}
\binom{n}{k}\bb{\tilde{U}_n(\X)-\tilde{U}_n(\X')} &= \sum_{S \in \mathcal{I}_{n,k}}\bb{g^{\X}(S)-g^{\X'}(S)} \notag \\
&= \underbrace{\sum_{S \cap B \neq \varnothing} \bb{g^{\X}(S)-g^{\X'}(S)}}_{T_1} + \underbrace{\sum_{\substack{i^* \notin S \\ S \cap B = \varnothing}} \bb{g^{\X}(S)-g^{\X'}(S)} }_{T_2} \notag\\
&~~~~ + \underbrace{\sum_{\substack{i^* \in S \\ S \cap B = \varnothing}} \bb{g^{\X}(S)-g^{\X'}(S)}}_{T_3}.
}
We bound each of the three terms separately. First, we show that the global sensitivity of $\buf{\X}$ is $1$.
\begin{lemma} \label{eq:bufX_sensitivity}
$|\buf{\X}-\buf{\X '}| \le 1.$
\end{lemma}
\begin{proof}
Note that 
\ba{\label{eq:Udiff}
\bmb{U_n(\X)-U_n(\X')} = \frac{1}{\binom{n}{k}} \bmb{\sum_{S \in \I^{i^*}_{n,k}} \bb{h(X_S) - h(X'_S)}} \le \frac{\binom{n-1}{k-1} C}{\binom{n}{k}} = \frac{kC}{n},
}
and for any $i \neq i^*$,
\ba{\label{eq:hhajekdiff}
\bmb{\h{\X}{X}{i}-\h{\X'}{X'}{i}} = \frac{1}{\binom{n-1}{k-1}} \bmb{\sum_{i,i^* \in S} \bb{h(X_S) - h(X'_S)}} \le \frac{\binom{n-2}{k-2} C}{\binom{n-1}{k-1}} \le \frac{kC}{n}.
}
Therefore, if an index $i \neq {i^*}$ is in $\Good(\X)$, then using Eqs~\eqref{eq:goodset},~\eqref{eq:Udiff}, and~\eqref{eq:hhajekdiff},
\ba{
\bmb{\h{\X'}{X'}{i}-U_n(\X')} &\le \bmb{\h{\X'}{X'}{i}-\h{\X}{X}{i}}+\bmb{\h{\X}{X}{i}-U_n(\X)}+\bmb{U_n(\X)-U_n(\X')} \label{eq:hu_triangle}\\
&\le \frac{kC}{n} + \bb{\conc +  \frac{2kC\buf{\X}}{n}} + \frac{kC}{n} = \conc +  \frac{2kC\bb{1+\buf{\X}}}{n} \notag,
}
which leaves at most $1+\buf{\X}$ potential indices $i$ for which $|\h{\X'}{X'}{i}-U_n(\X')| > \conc +\frac{2kC(1+\buf{\X})}{n}$: the indices in $\Bad(\X)$ and the index ${i^*}$. Therefore, $\buf{\X'} \le \buf{\X}+1$. Similarly, $\buf{\X} \le \buf{\X'}+1$.
\end{proof}
From Eqs~\eqref{eq:Udiff} and~\eqref{eq:hhajekdiff}, $\bmb{\h{\X'}{X'}{i}-U_n(\X')} - \bmb{\h{\X}{X}{i}-U_n(\X)} \le \frac{2kC}{n}$ for $i \neq i^*$, which immediately implies the following lemma:
\begin{lemma}\label{lem:weight_sensitivity}
For all $i \neq i^*$, $\bmb{\wt^\X(i)-\wt^{\X'}(i)} \le \frac{2kC\beta}{n}$.
\end{lemma}

\paragraph{Bounding the first term:} To bound the term $T_1$ in~\eqref{eq:sum_decomp}, we decompose it further as
\ba{\label{eq:T1_decomp}
T_1 &= \sum_{i \in B} \sum_{S \in \I^i_{n,k}} \bb{g^{\X}(S)-g^{\X'}(S)} - \sum_{a=2}^{k} \sum_{|S \cap B| = a} (a-1) \bb{g^{\X}(S)-g^{\X'}(S)} \notag\\
&= \binom{n-1}{k-1} \sum_{i \in B} \bb{\g{\X}{X}{i}-\g{\X'}{X'}{i}} - \sum_{a=2}^{k} \sum_{|S \cap B| = a} (a-1) \bb{g^{\X}(S)-g^{\X'}(S)}.
}
The first term sums over all subsets that contain some element in $B$. However, this leads to over-counting every subset with $a$ elements in common with $B$ exactly $a-1$ times. The second term corrects for this over-counting, akin to an inclusion-exclusion argument.

Consider any index $i \in B$. If $\bmb{\h{\X}{X}{i} - U_n(\X)} \ge \conc + \frac{2kC\bb{2+\buf{\X}}}{n} + \frac{1}{\beta}$, then from equations~\ref{eq:Udiff} and~\ref{eq:hhajekdiff}, $\bmb{\h{\X'}{X'}{i} - U_n(\X')} \ge \conc + \frac{2kC\bb{1+\buf{\X}}}{n} + \frac{1}{\beta} \ge \conc + \frac{2kC\buf{\X'}}{n} + \frac{1}{\beta}$, so $\wt_\X(i) = \wt_{\X'}(i) = 0$. In this case, $\bmb{\g{\X}{X}{i}-\g{\X'}{X'}{i}} = \bmb{U_n(\X)-U_n(\X')} \le \frac{kC}{n}$. Otherwise, $\bmb{\h{\X}{X}{i} - U_n(\X)} < \conc + \frac{2kC\bb{2+\buf{\X}}}{n} + \frac{1}{\beta}$. Now,
\ba{\label{eq:g_decomp}
\sum_{S \in \I^i_{n,k}} g^{\X}(S) &= \sum_{S \in \I^i_{n,k}} \bb{h(X_S)\wt^\X(S) + U_n(\X)\bb{1-\wt^\X(S)}} \notag \\
&= \sum_{S \in \I^i_{n,k}} \bb{h(X_S)\wt^\X(i) + U_n(\X)\bb{1-\wt^\X(i)}} \notag \\
&~~+\sum_{S \in \I^i_{n,k}} \bb{h(X_S)- U_n(\X)}\bb{\wt^\X(S)-\wt^\X(i)}.
}
The first term in the sum above is equal to $\binom{n-1}{k-1}\bb{(\h{\X}{X}{i}-U_n)\wt^\X(i) + U_n(\X)}$, which we bound as follows:


For the second term, if $i$ has the minimum weight among the indices in $S$, then $\wt^\X(S)=\wt^\X(i)$. Otherwise, some index $j \in S$ is such that $\wt^\X(j) < \wt^\X(i)$. Note that such an index $j$ is necessarily in $\Bad(\X)$ because its weight is less than $1$. If $i^* \notin S$, then
\bas{
\bmb{h(X'_S) - U_n(\X')} - \bmb{h(X_S) - U_n(\X)} \le \bmb{U_n(\X)-U_n(\X')} = \frac{kC}{n},
}
and by lemma~\ref{lem:weight_sensitivity}, \bas{
\bmb{\wt^{\X'}(S)-\wt^{\X'}(i)}-\bmb{\wt^\X(S)-\wt^\X(i)} \le \frac{4kC\beta}{n}.
}
There are at most $\binom{n-1}{k-1}-\binom{n-1-\buf{\X}}{k-1}$  sets $S$ that contain $i$ and some index $j \neq i$ such that $j \in \Bad(\X)$. Moreover, there are at most $\binom{n-2}{k-2}$ sets $S$ that contain $i$ and $i^*$. Using these bounds in~\ref{eq:g_decomp}, and
the bounds from~\ref{eq:Udiff},~\ref{eq:hhajekdiff}, and lemma~\ref{lem:weight_sensitivity}, we bound the first term of~\ref{eq:T1_decomp} as
\ba{\label{eq:T11_bound}
\bmb{\g{\X}{X}{i}-\g{\X'}{X'}{i}} &\le \bb{\conc + \frac{2kC\bb{3+\buf{\X}}}{n}+\frac{1}{\beta}}\frac{2kC\beta}{n} + \frac{3kC}{n} \notag \\
&+ \frac{\binom{n-1}{k-1}-\binom{n-1-\buf{\X}}{k-1}}{\binom{n-1}{k-1}} \bb{\frac{kC}{n} + \frac{2kC\beta}{n} C} + \frac{\binom{n-2}{k-2}}{\binom{n-1}{k-1}}C \notag \\
% \bb{\conc + \frac{2kC\bb{3+\buf{\X}}}{n}+\frac{1}{\beta}}\frac{2kC\beta}{n}+\frac{2kC}{n}+\frac{kC}{n}+\frac{2kC\buf{\X}}{n}+\frac{2kC\buf{\X'}}{n} \notag \\
&\le \bb{\conc + \frac{2kC\bb{3+2\buf{\X}}}{n}}\frac{2kC\beta}{n} + \frac{kC\bb{6+\frac{2k\buf{\X}}{n}}}{n},
% &\le \bb{\conc + \frac{2kC\bb{3+\buf{\X}}}{n}}\frac{2kC\beta}{n} + \frac{kC\bb{7+4\buf{\X}}}{n},
}
where we used
\bas{
\frac{\binom{n-1}{k-1} - \binom{n-1-\buf{\X}}{k-1}}{\binom{n-1}{k-1}} = 1 - \prod_{t=1}^{k-1} \bb{1 - \frac{\buf{\X}}{n-t}} %\le 1 - \bb{1 - \frac{\buf{\X}}{n-k+1}}^{k-1} \\
\le 1 - \bb{1-\frac{(k-1)\buf{\X}}{n-k+1}} \le \frac{2k\buf{\X}}{n}.
}
For the second term of~\ref{eq:T1_decomp}, consider any set $S$ such that $i^* \notin S$. Then, using $\bmb{\wt^\X(S)-\wt^{\X'}(S)} \le \frac{2kC\beta}{n}$ and $\bmb{\h{\X'}{X'}{i}-U_n(\X')} - \bmb{\h{\X}{X}{i}-U_n(\X)} \le \frac{2kC}{n},$
\bas{
g^{\X}(S) - g^{\X'}(S) \le C \cdot \frac{2kC\beta}{n} + \frac{2kC}{n} \cdot 1 + \frac{kC}{n} = \frac{2kC\beta}{n}C + \frac{3kC}{n}.
}
So,
\ba{
&\frac{1}{\binom{n}{k} \bb{\frac{2kC\beta}{n}C + \frac{3kC}{n}}} \bmb{\sum_{a=2}^{k} \sum_{\substack{\bmb{S \cap B} = a \\ i^* \notin S}} (a-1)\bb{g^{\X}(S)-g^{\X'}(S)}} \notag \\
&\le \frac{1}{\binom{n}{k}}\sum_{a=2}^k (a-1)\binom{b}{a}\binom{n-1-b}{k-a} \le \frac{1}{\binom{n}{k}}\sum_{a=2}^k (a-1)\binom{b}{a}\binom{n-b}{k-a} \notag\\
&\le \frac{\binom{n-b}{k}}{\binom{n}{k}} - \bb{1 - \frac{bk}{n}} \le \bb{1 - \frac{b}{n}}^k - \bb{1-\frac{bk}{n}} \le \frac{b^2k^2}{n^2} \le \frac{k^2(2\buf{\X}+1)^2}{n^2} \notag,
}
where we used the identities 
\bas{
\sum_{a=0}^k \binom{b}{a}\binom{n-b}{k-a} = \binom{n}{k}, \qquad \sum_{a=0}^k a\binom{b}{a}\binom{n-b}{k-a} = \frac{bk}{n}\binom{n}{k}.
}
Moreover,
\ba{
\frac{1}{C}\bmb{ \frac{1}{\binom{n}{k}} \sum_{a=2}^{k} \sum_{\substack{\bmb{S \cap B} = a \\ i^* \in S}} (a-1)\bb{g^{\X}(S)-g^{\X'}(S)}} &\le \frac{1}{\binom{n}{k}} \sum_{a=2}^{k-1} (a-1)\binom{b}{a}\binom{n-1-b}{k-1-a} \notag \\
&\le \frac{k}{n} \frac{b^2(k-1)^2}{(n-1)^2} \le \frac{k^3 (2\buf{\X}+1)^2}{n^3} \notag
}
Combining the above two bounds, we get
\ba{\label{eq:T12_bound}
\frac{1}{\binom{n}{k}}\sum_{a=2}^{k} \sum_{|S \cap B| = a} (a-1) \bb{g^{\X}(S)-g^{\X'}(S)}
&\le \frac{k^2(2\buf{\X}+1)^2}{n^2}\bb{\frac{2kC\beta}{n}C+ \frac{4kC}{n}}.
}
Using the bounds from~\ref{eq:T11_bound} and~\ref{eq:T12_bound},
\bas{
\frac{1}{\binom{n}{k}} \bmb{T_1} &\le \frac{k}{n}\bb{\bb{\conc + \frac{2kC\bb{3+2\buf{\X}}}{n}}\frac{2kC\beta}{n} + \frac{kC\bb{6+\frac{2k\buf{\X}}{n}}}{n}}\bmb{B} +\frac{k^2(2\buf{\X}+1)^2}{n^2}\bb{\frac{2kC\beta}{n}C+ \frac{4kC}{n}} \\
&\le \frac{2k^2C\beta}{n^2}\bb{\conc + \frac{2kC\bb{7+6\buf{\X}}}{n}}\bb{2\buf{\X}+1} + \frac{k^2C}{n^2}\bb{6 + \frac{k\bb{4\buf{\X}+1}}{n}}\bb{2\buf{\X}+1}
}
Next, we bound the second term of~\ref{eq:sum_decomp}.  This sum is simply $0$: for any $S \subseteq G$, the weight of any index in $G$ is $1$ in both $\X$ and $\X'$, and $h(X_S) = h(X'_S)$ for any such $S$. It remains to bound the third term, $T_3$, of~\ref{eq:sum_decomp}.
If $\wt^{\X}(i^*) = 0$, then $\g{\X}{X_{i^*}}{{i^*}} = U_n(\X)$. Otherwise, from equation~\ref{eq:g_decomp},
\bas{
\bmb{\g{\X}{X_{i^*}}{{i^*}}-U_n(\X)} \le \bmb{\h{\X}{X}{i^*}-U_n(\X)} + \frac{\binom{n-1}{k-1}-\binom{n-1-\buf{\X}}{k-1}}{\binom{n-1}{k-1}} C \le \conc + \frac{2kC\bb{1+2\buf{\X}}}{n} + \frac{1}{\beta}.
}
Either way, $\g{\X}{X_{i^*}}{{i^*}}$ is within $\frac{2kC\bb{1+2\buf{\X}}}{n} + \frac{1}{\beta}$ of $\conc$. Note that the sum in $T_3$ runs only over $i^* \in S$ that do not intersect with $B$. The number of sets $S$ containing both $i^*$ and some element of $B$ is bounded by $\binom{n-2}{k-2}|B|$, which means we can bound $T_3$ as
\ba{
\frac{1}{\binom{n}{k}} |T_3| &\le \frac{k}{n} \bb{\conc + \frac{2kC\bb{1+2\buf{\X}}}{n} + \frac{1}{\beta}} + \frac{\binom{n-2}{k-2}}{\binom{n}{k}}\bb{2\buf{\X}+1}C \notag\\
&\le \frac{k}{n} \bb{\conc + \frac{3kC\bb{1+2\buf{\X}}}{n} + \frac{1}{\beta}}.
}

Combining the bounds on $T_1, T_2, $ and $T_3$ in~\ref{eq:sum_decomp}, we conclude
\bas{
\bmb{\tilde{U}_n(\X) - \tilde{U}_n(\X')} = O\bb{ \frac{k}{n}\bb{\conc + \frac{kC\buf{\X}}{n}}\bb{1 + \frac{kC\buf{\X}\beta}{n}} + \frac{k}{n\beta} + \frac{k^3 \buf{\X}^2}{n^3}C},
}
which implies that
\ba{\label{eq:local_bound}
LS_{\tilde{U}_n}(\X) = O\bb{ \frac{k}{n}\bb{\conc + \frac{kC\buf{\X}}{n}}\bb{1 + \frac{kC\buf{\X}\beta}{n}} + \frac{k}{n\beta} + \frac{k^3 \buf{\X}^2}{n^3}C }
}
for some universal constant; for the sake of simplicity, assume this constant is $1$. Let $g(\conc ,\buf{\X},n) := \frac{k}{n}\bb{\conc + \frac{kC\buf{\X}}{n}}\bb{1 + \frac{kC\buf{\X}\beta}{n}} + \frac{k}{n\beta} + \frac{k^3 \buf{\X}^2}{n^3}C$; note that it is strictly increasing in $\buf{\X}$. Define
\ba{\label{eq:smooth_sensitivity}
S(G) = \max_{\ell \in \mathbb{Z}_{\ge 0}} e^{-\epsilon \ell} g(\conc , \buf{\X}+\ell, m).
}
\begin{lemma}\label{lem:smooth_bound}
$S(G)$ is an $\epsilon$-smooth upper bound on $LS_f(G)$. Moreover,
\[S(G) = O\bb{ \frac{k}{n}\bb{\conc + \frac{kC\bb{\buf{\X}+1/\epsilon}}{n}}\bb{1 + \frac{kC\bb{\buf{\X}+1/\epsilon}\beta}{n}} + \frac{k}{n\beta} + \frac{k^3 \bb{\buf{\X}+1/\epsilon}^2}{n^3}C }.\]
\end{lemma}
% \begin{proof}[Proof of Lemma~\ref{lem:smooth_bound}]
% Clearly, $S(G) \ge g(\conc , \buf{\X}, n) \ge LS_f(G)$, and for any two adjacent $G$ and $G'$,
% \bas{
% S(G') &= \max_{\ell \in \mathbb{Z}_{\ge 0}} e^{-\epsilon \ell} g(\conc , \buf{\X'}+\ell, n) \le \max_{\ell \in \mathbb{Z}_{\ge 0}} e^{-\epsilon \ell} g(\conc , \buf{\X}+\ell+1, n) \\
% &= \max_{\ell \in \mathbb{Z}_{> 0}}e^{-\epsilon \bb{\ell-1}} g(\conc , \buf{\X}+\ell+1, n) \le e^{\epsilon}\max_{\ell \in \mathbb{Z}_{\ge 0}}e^{-\epsilon\ell} g(\conc , \buf{\X}+\ell+1, n) = e^{\epsilon}S(G).
% }
% This shows that $S$ is an $\epsilon$-smooth upper bound on the local sensitivity of $f$. As for the upper bound, for any $\ell \ge 0$, we have
% \bas{
% e^{-\epsilon\ell}g(\conc , \buf{\X}+\ell, n) &= e^{-\epsilon\ell} \frac{4k\bb{\buf{\X}+\ell}}{n} \bb{2\conc  + \frac{17k\bb{\buf{\X}+\ell}}{n-1}C} \\
% &= \frac{4k\bb{\buf{\X}e^{-\epsilon\ell/2}+\ell e^{-\epsilon\ell/2}}}{n} \bb{2\conc  e^{-\epsilon\ell/2} + \frac{17k\bb{\buf{\X}e^{-\epsilon\ell/2}+\ell e^{-\epsilon\ell/2}}}{n-1}C} \\
% &\le \frac{4k\bb{\buf{\X}+1/\epsilon}}{n}\bb{2\conc   + \frac{17k\bb{\buf{\X}+1/\epsilon}}{n-1}C}.
% }
% \end{proof}

By Lemma~\ref{lem:smooth_bound}, it is clear that the term $S(\X)$ added in to $\tilde{U}_n(\X)$ in Algorithm~\ref{alg:PrivateMeanDegenerate} is exactly the smoothed sensitivity defined in Eq~\ref{eq:smooth_sensitivity}. Therefore, the output $\tilde{U}_n(\X)+S(\X)/\epsilon \cdot Z$, where $Z$ is sampled from a Student's $t$-distribution with three degrees of freedom, is $\epsilon$-differentially private. 

\paragraph{Utility.}First, by Chebyshev's inequality, we have with probability at least $1-\alpha$ that
$\bmb{U_n(\X)-\theta} \le \frac{1}{\sqrt{\alpha}}\sqrt{\Var(U_n)}.
$
Second, with probability at least $1-\alpha$ the estimate $\tilde{\zeta}_k$ of the variance of $h$ satisfies $\zeta_k \le \tilde{\zeta}_k \le 2\zeta_k$. 
First note that since $\Var(h(X_1,\dots,X_k|X_i)) = \zeta_1 = 0$, we have $\E[h(X_1, \dots, X_k)|X_i] = \E[h(X_1, \dots, X_k)] = \theta$. %Also, since
% $\sigma_i^2  \le \E\bbb{\bb{h(X_S)-\theta}^2|X_i}$

Next, note that $\sigma_i^2$ are IID subexponential random variables with subexponential norm at most $K\zeta_k$, because by Jensen's inequality,
$
\E\bbb{\exp \bb{t\sigma_i^2}} % &= \E\bbb{\exp \bb{t\Var{\bb{h(X_S) | X_1}}}}
%&= \E\bbb{\exp\bb{t \E\bbb{\bb{h(X_S)-\theta}^2 \big| X_1}}} \\
%&\le \E\bbb{\E \bbb{\exp\bb{t \bb{h(X_S)-\theta}^2 } \big| X_1}} \\
\leq \E \bbb{\exp\bb{t \bb{h(X_S)-\theta}^2 } }.
$
Conditioned on this event, and using Lem~\ref{lem:degen_conc_hajek}, with probability at least $1-\alpha$, all $\h{\X}{X}{i}$ satisfy
\vspace{-1em}
\bas{
\bmb{\h{\X}{X}{i}-\theta} \le \bb{2\sqrt{\frac{4kK}{n}}\sqrt{\tilde{\zeta}_k} + \frac{4k}{3n}C}\log \frac{12n}{\alpha} \le \frac{\conc}{2}.
}
\vspace{-.3em}
Moreover, each of the projections $\h{\X}{X}{i}$ is within $\conc/2$ of the true mean $\theta$  with probability at least $1-\alpha$. If so, then each of the projections is also within $\conc$ of the empirical mean of the projections. This means $\Good(\X) = [n]$ and $\buf{\X} = 1$. Also, since all indices are good, $g^{\X}(S) = h(X_S)$ for all $S$ and $\tilde{U}_n(\X) = U_n(\X)$.
Finally, with probability at least $1-\alpha,$ the $Z$ satisfies
$Z \le \frac{1}{\sqrt{\alpha}} \Var(t_3) = \frac{3}{\sqrt{\alpha}}.$
Therefore,
\vspace{-1em}
\ba{\label{eq:degen:error}
&\bmb{\mathcal{A}(\X)-\theta} \le \bmb{\tilde{U}_n(\X)-U_n(\X)}+\bmb{U_n(\X)-\theta}+\bmb{S(\X)/\epsilon \cdot Z} \notag\\
&\le 0 + \frac{1}{\sqrt{\alpha}}\sqrt{\Var(U_n)} + \frac{3}{\epsilon \sqrt{\alpha}} \frac{4k\bb{1+1/\epsilon}}{n}\bb{2\conc   + \frac{17k\bb{1+1/\epsilon}}{n-1}C} \\
&= O\bb{\sqrt{\Var(U_n)} + 
\frac{k^{3/2} \sqrt{K} \bb{1+1/\epsilon} \log n}{n^{3/2}\epsilon}\sqrt{\zeta_k}  + \frac{k^2 \bb{1+1/\epsilon}^2 \log n}{n^2\epsilon}C}
}
conditioned on all the aforementioned events, which occur with probability $0.99$.
\end{proof}

==> setup_old.tex <==
% \input{macros.tex}
% \begin{algorithm}
% \caption{\label{alg:MedianOfMeans} \textbf{Median of Means}$\bb{n, k, h, \left \{X_i \right\}_{i \in [n]}, \F= \{\I_1, \dots, \I_m\}, R, \eps, \alpha, \Yc{}, \Uc{}}$}
% \begin{algorithmic}[1]
% % \STATE Let $\F $
% \STATE $t \gets \log\bb{R/\Uc{\alpha}}$
% \STATE $[l_0, r_0] \gets [-R,R]$
% \FOR{$j = 1, \dots, m$}
% \STATE $Y_{0,j} \gets \frac{1}{\bmb{\I_j}}\sum_{S \in \I_j} h(X_S)$
% \ENDFOR
% % \STATE $\{Y_{0,j}\}_{j \in [m]} \gets \text{GenerateYFromX}\bb{n, \{X_i\}_{i \in [n]}}$
% % \STATE $\eps' \gets \eps/2t, \beta \gets \alpha/t$
% \FOR{$i = 1,2,...,t$}
% \STATE $\{Y_{i,j}\}_{j \in [m]}, [l_i, r_i] \gets \text{U-StatOneStep}\bb{n, k, \{Y_{i-1, j}\}, \F, [l_{i-1}, r_{i-1}], \eps/2t, \alpha/t, \Yc{}, \Uc{}}$ 
% % \COMMENT{{\rd $Y_i$ may change after each call, because it is truncated in each step and this truncated value is used in the subsequent calls}}
% \ENDFOR
% \STATE $\{Y_{t+1,j}\}_{j \in [m]}, [l_{t+1}, r_{t+1}] \gets \text{U-StatOneStep}\bb{n, k, \{Y_{t,j}\}, \F, [l_t, r_t], \eps/2, \alpha/2, \Yc{}, \Uc{}}$
% \RETURN $(l_{t+1}+r_{t+1})/{2}$
% \end{algorithmic}
% \end{algorithm}


% \purna{move below to notation}
% \begin{definition}
% (Clipping) For any $l,r \in \mathbb{R}$ with $l \le r$, we define the clipping of a real number $x$ in the interval $[l,r]$ as
% \[\proj_{l,r}\bb{x} = \max\bb{l, \min\bb{x,r}}. \]
% \end{definition}

% \textcolor{red}{PL: Is it possible to apply the ``mother theorem" also to heavy-tailed data, by using a median-of-means trick? We need concentration of individual $Y_i$'s, as well as the average of all of them. If we were to compute each of the $Y_i$'s by chunking up the data and taking a median of means, perhaps we could get away with just assuming $2+\delta$ moments, rather than sub-exponential tails?}
% \textcolor{blue}{Perhaps it works. I don't know how to argue about the concentration of the mean of the medians.}
In Algorithms~\ref{alg:PrivateMean} and~\ref{alg:OneStep}, we present a natural extension of the Coinpress algorithm~\citep{biswas2020coinpress}, which is then used to obtain a private estimate of $\theta$ with the non-private term matching $\Var(U_n)$. Originally, this algorithm was used for private mean and covariance estimation of IID (sub)Gaussian data. Our idea allows us to extend the algorithm to take as input the data $\{Y_j\}_{j \in [m]}$ such that (i) each $Y_j$ is equal to $h(X_S)$ for some $S$, (ii) the $Y_j$'s are \textit{weakly dependent} on each other, and (iii) each $Y_j$, as well as their mean $\sum_{j \in [m]} Y_j/m$, has sufficiently strong concentration around the population mean. 

For instance, suppose $m = \lfloor n/k \rfloor$ and $Y_j = h(X_{S_j})$ for all $j \in [m]$, where $S_j = \{(j-1)k+1, \dots, (j-1)k+k \}$. Then, Algorithm~\ref{alg:PrivateMean} reduces to the Coinpress algorithm applied to $n/k$ independent data.
% Our goal is to provide a private estimator for an unknown, estimable parameter $\theta$. We begin by introducing a simple non-private estimator that estimates $\theta$ by an average of independent quantities:
% \begin{definition}[Naive family]\label{def:naive}
% Let $m=\lfloor n/k \rfloor$ and $\I_j \defeq \{ \{(j-1)k+1, \dots, (j-1)k+k \} \}$ for all $j \in [m]$. Define $\F_{\text{naive}} = \{\I_1, \dots, \I_m\}$, which we call the ``naive'' family.
% \end{definition}
% Estimate $\theta$ using $\tn \defeq \frac{1}{m} \sum_{i=1}^{m} h(X_{(j-1)k+1}, \dots, X_{(j-1)k+k})$.
\begin{remark}
\label{RemNaive} 
All existing private mean estimation algorithms \citep{KV18, KSSU19, KLSU19, biswas2020coinpress} applied to the $n/k$ IID values $h(X_{S_1}), h(X_{S_2}), \dots, h(X_{S_{n/k}})$ provide a confidence interval of width
\bas{
O\bb{\sqrt{\Var\bb{\hat{\theta}_{\text{naive}}}} + \frac{k\sqrt{\zeta_k}}{n\epsilon}} = O\bb{\underbrace{\sqrt{\frac{k\zeta_k}{n}}}_{\text{non-private error}} + \underbrace{\frac{k\sqrt{\zeta_k}}{n\epsilon}}_{\text{private error}}},
}
using the relation $\Var\bb{\tn}=k\zeta_k/n$, where $\zeta_k$ is defined in Eq~\ref{eq:condvar}. Note that this variance term is larger than the dominant term $k^2\zeta_1/n$ of $\Var(U_n)$ (see Lemma~\ref{lem:Ustatvar} and Eq~\ref{eq:varhierarchy}), which stems from the fact that the naive estimator is a sub-optimal estimator of $\theta$. The optimal estimator is the U statistic defined in Eq~\ref{eq:ustat} (see Chapter 1, Theorem 3 of \citep{Lee1990UStatisticsTA}). 
\end{remark}
% In Algorithms~\ref{alg:PrivateMean} and~\ref{alg:OneStep}, we present a general extension of the Coinpress algorithm~\citep{biswas2020coinpress}, which is then used to obtain a private estimate of $\theta$ with the non-private term matching $\Var(U_n)$. Originally, this algorithm was used for private mean and covariance estimation of i.i.d.\ (sub)-Gaussian data. Our idea allows us to extend the algorithm to take as input the data $\{Y_j\}_{j \in [m]}$ such that (i) each $Y_j$ is a (weighted) linear combination of the $h(X_S)$ with $\E\bbb{Y_j} = \theta$, (ii) the $Y_j$'s are \textit{weakly dependent} on each other, and (iii) the $Y_j$'s, and their mean $\sum_{j \in [m]} Y_j/m$, each has sufficiently strong concentration around the population mean $\theta$. We formalize this idea next.

\begin{algorithm}
\caption{\label{alg:PrivateMean} \textbf{U-StatMean}$\bb{n, k, h, \left \{X_i \right\}_{i \in [n]}, \F= \{S_1, \dots, S_m\}, R, \eps, \alpha, \Yc{.}, \Uc{.}}$}
\begin{algorithmic}[1]
% \STATE Let $\F $
% \STATE \textcolor{red}{should $\alpha$ be a general input?}
% \textcolor{blue}{we can let $\alpha$ be a general input, which will give us a $\frac{1}{\sqrt{\alpha}} \var(U_n)$ error. We can later pick $\alpha = 0.01$ and apply the median-of-means trick.}
\STATE $t \gets \log\bb{R/\Yc{\alpha}}, \; [l_0, r_0] \gets [-R,R]$
\FOR{$j = 1, \dots, m$}
\STATE $Y_{0,j} \gets \frac{1}{\bmb{\I_j}}\sum_{S \in \I_j} h(X_S)$
\ENDFOR
% \STATE $\{Y_{0,j}\}_{j \in [m]} \gets \text{GenerateYFromX}\bb{n, \{X_i\}_{i \in [n]}}$
% \STATE $\eps' \gets \eps/2t, \beta \gets \alpha/t$
\FOR{$i = 1,2,...,t$}
\STATE $\{Y_{i,j}\}_{j \in [m]}, [l_i, r_i] \gets \text{U-StatOneStep}\bb{n, k, \{Y_{i-1, j}\}, \F, [l_{i-1}, r_{i-1}], \eps/2t, \alpha/t, \Yc{.}, \Uc{.}}$ 
% \COMMENT{{\rd $Y_i$ may change after each call, because it is truncated in each step and this truncated value is used in the subsequent calls}}
\ENDFOR
\STATE $\{Y_{t+1,j}\}_{j \in [m]}, [l_{t+1}, r_{t+1}] \gets \text{U-StatOneStep}\bb{n, k, \{Y_{t,j}\}, \F, [l_t, r_t], \eps/2, \alpha, \Yc{.}, \Uc{.}}$
\RETURN $(l_{t+1}+r_{t+1})/{2}$
\end{algorithmic}
\end{algorithm}
\rd
\begin{remark}
    Note that one can rewrite Algorithm~\ref{alg:PrivateMean} with $\alpha$ as a general input. However, we set $\alpha=0.01$ so that later, the median of means type approach can be applied to boost the error probability. We pass $\Yc{.}$  ( $\Uc{.}$), which is a function whose form is governed by the uniform concentration of $Y_i$'s ($\sum_{j=1}^m Y_j/m$). For example, if $Y_i's$ are sub-gaussian with variance proxy one, then $\Yc{x}= \sqrt{\log m/x}$.
\end{remark}
\bk
\begin{algorithm}
\caption{\label{alg:OneStep} \textbf{U-StatOneStep}$\bb{n, k, \left\{Y_i \right\}_{i \in [m]}, \F, [l,r], \eps', \beta, \Yc{.}, \Uc{.}}$}
\begin{algorithmic}[1]
\STATE $Y_j \gets \proj_{l-\Yc{\beta}, r+\Yc{\beta}}\bb{Y_j}$ for all $1 \le j \le m$.
% \STATE Let $\Delta$ be the sensitivity of $\frac{1}{m} \sum_{i=1}^m Y_i$.
\STATE $\Delta \gets \dep{n}{k}{\F}\bb{r-l+2\Yc{\beta}}$
\STATE $Z \gets \frac{1}{m} \sum_{j=1}^{m} Y_j + W$, where $W \sim \text{Lap}\bb{\frac{\Delta}{\eps'}}$
\STATE $[l,r] \gets \bbb{Z - \bb{\Uc{\beta}+\frac{\Delta}{\eps'} \log \frac{1}{\beta}}, Z + \bb{\Uc{\beta}+\frac{\Delta}{\eps'} \log \frac{1}{\beta}}}$
\RETURN $\{Y_j\}_{j \in [m]}, [l,r]$ 
\end{algorithmic}
\end{algorithm}

% \begin{algorithm}
% \caption{\label{alg:PrivateMean} \textbf{U-StatMean}$\bb{n, k, h, \left \{X_i \right\}_{i \in [n]}, \F= \{\I_1, \dots, \I_m\}, R, \eps, \Yc{}, \Uc{}}$}
% \begin{algorithmic}[1]
% % \STATE Let $\F $
% \STATE \textcolor{red}{should $\alpha$ be a general input?} $\alpha \gets 0.01, \; t \gets \log\bb{R/\Yc{}}, \; [l_0, r_0] \gets [-R,R]$
% \FOR{$j = 1, \dots, m$}
% \STATE $Y_{0,j} \gets \frac{1}{\bmb{\I_j}}\sum_{S \in \I_j} h(X_S)$
% \ENDFOR
% % \STATE $\{Y_{0,j}\}_{j \in [m]} \gets \text{GenerateYFromX}\bb{n, \{X_i\}_{i \in [n]}}$
% % \STATE $\eps' \gets \eps/2t, \beta \gets \alpha/t$
% \FOR{$i = 1,2,...,t$}
% \STATE $\{Y_{i,j}\}_{j \in [m]}, [l_i, r_i] \gets \text{U-StatOneStep}\bb{n, k, \{Y_{i-1, j}\}, \F, [l_{i-1}, r_{i-1}], \eps/2t, \alpha/t, \Yc{}, \Uc{}}$ 
% % \COMMENT{{\rd $Y_i$ may change after each call, because it is truncated in each step and this truncated value is used in the subsequent calls}}
% \ENDFOR
% \STATE $\{Y_{t+1,j}\}_{j \in [m]}, [l_{t+1}, r_{t+1}] \gets \text{U-StatOneStep}\bb{n, k, \{Y_{t,j}\}, \F, [l_t, r_t], \eps/2, \alpha, \Yc{}, \Uc{}}$
% \RETURN $(l_{t+1}+r_{t+1})/{2}$
% \end{algorithmic}
% \end{algorithm}

% \begin{algorithm}
% \caption{\label{alg:OneStep} \textbf{U-StatOneStep}$\bb{n, k, \left\{Y_i \right\}_{i \in [m]}, \F, [l,r], \eps', \beta, \Yc{}, \Uc{}}$ \textcolor{red}{change all $Q_\beta$'s to $Q$?}}
% \begin{algorithmic}[1]
% \STATE $Y_j \gets \proj_{l-\Yc{\beta}, r+\Yc{\beta}}\bb{Y_j}$ for all $1 \le j \le m$.
% % \STATE Let $\Delta$ be the sensitivity of $\frac{1}{m} \sum_{i=1}^m Y_i$.
% \STATE $\Delta \gets \dep{n}{k}{\F}\bb{r-l+2\Yc{\beta}}$
% \STATE $Z \gets \frac{1}{m} \sum_{j=1}^{m} Y_j + W$, where $W \sim \text{Lap}\bb{\frac{\Delta}{\eps'}}$
% \STATE $[l,r] \gets \bbb{Z - \bb{\Uc{\beta}+\frac{\Delta}{\eps'} \log \frac{1}{\beta}}, Z + \bb{\Uc{\beta}+\frac{\Delta}{\eps'} \log \frac{1}{\beta}}}$
% \RETURN $\{Y_j\}_{j \in [m]}, [l,r]$ 
% \end{algorithmic}
% \end{algorithm}


\paragraph{Setup.} Let $n$ and $k$ be positive integers such that $k \le n/2$. Let $m = m_{n,k}$ be a positive integer and let $\F = \F_{n,k} = \bcb{\I_1, \I_2, \dots, \I_m}$ be a family of non-empty subsets of $\I_{n,k}$, not necessarily distinct. For each $i \in [n]$, let
\ba{\label{eq:index_frac}
f_i \defeq \frac{\bmb{\bcb{j \in [m]: \exists~S \in \I_j \text{ such that } i \in S}}}{m}
}
be the fraction of indices $j$ such that $\I_j$ ``depends'' on the index $i$, and define
\ba{\label{eq:dep_n_k}
\dep{n}{k}{\mathcal{F}} \defeq \max_{i \in [n]} f_i.
}
Let $h: \mathcal{X}^k \to \mathbb{R}$ be a symmetric function and let $\mathcal{D}$ be an unknown distribution over $\mathcal{X}$ with $\E\bbb{h(\mathcal{D}^k)} = \theta$.
For each $j \in [m]$, let $Y_j \defeq \frac{1}{|I_j|} \sum_{S \in \I_j} h(X_S).$ Clearly, $\E\bbb{Y_j} = \theta$. Moreover, $\dep{n}{k}{\mathcal{F}}$ is an upper bound on the fraction of $Y_j$ that change if any single $X_i$ is changed. To allow for small noise addition while ensuring privacy, it is desirable to choose $\mathcal{F}$ such that $\dep{n}{k}{\mathcal{F}}$ is small.

Define $\Yc{\beta} = Q_{n,k,h,\mathcal{D}, \mathcal{F}}(\beta)$ and $\Uc{\beta} = Q^{\text{avg}}_{n,k,h,\mathcal{D}, \mathcal{F}}(\beta)$ for all $\beta \in (0,1]$ such that
%for all $j \in [m]$, $\beta$ is an upper bound on the probability that $|Y_j-\theta|$ exceeds $\Yc{\beta}$, that is, for all $j \in [m]$,
\ba{\label{eq:def_yc_uc}\mathbb{P}\bb{\sup_{j \in [m]} \bmb{Y_j-\theta} > \Yc{\beta}} < \beta, \text{ and }
\mathbb{P}\bb{\bmb{\frac{1}{m}\sum_{j=1}^m Y_j - \theta} > \Uc{\beta}} < \beta.}
% } Also, let $\Uc{\beta} = \Uc{\beta}\bb{n,k,h,\mathcal{D}, \mathcal{F}}$ be defined such that
% \ba{\label{eq:def_uc} \mathbb{P}\bb{\bmb{\frac{1}{m}\sum_{j=1}^m Y_j - \theta} > \Uc{\beta}} < \beta.}
We will refer to $\Yc{\beta}$ and $\Uc{\beta}$ as $\beta$-\textit{confidence bounds} for $\sup_{j \in [m]} \bmb{Y_j - \theta}$ and $\bmb{\frac{1}{m}\sum_{j \in [m]} Y_j - \theta}$ respectively. Finally, let $\text{size}\bb{\F} \defeq \sum_{j \in [m]} |\I_j|$.
\textcolor{red}{It's not clear from the description whether the bounds~\eqref{eq:def_yc_uc} need to hold for all $\beta$ (probably not) or just a collection of $\beta$'s related to $\alpha$.} \textcolor{blue}{yes, we only need it for those specific $\alpha$ and $\beta$s related to $\alpha$.}


